On discretisation drift and smoothness regularisation in neural network training

The deep learning recipe of casting real-world problems as mathematical optimisation and tackling the optimisation by training deep neural networks using gradient-based optimisation has undoubtedly proven to be a fruitful one. The understanding behind why deep learning works, however, has lagged behind its practical significance. We aim to make steps towards an improved understanding of deep learning with a focus on optimisation and model regularisation. We start by investigating gradient descent (GD), a discrete-time algorithm at the basis of most popular deep learning optimisation algorithms. Understanding the dynamics of GD has been hindered by the presence of discretisation drift, the numerical integration error between GD and its often studied continuous-time counterpart, the negative gradient flow (NGF). To add to the toolkit available to study GD, we derive novel continuous-time flows that account for discretisation drift. Unlike the NGF, these new flows can be used to describe learning rate specific behaviours of GD, such as training instabilities observed in supervised learning and two-player games. We then translate insights from continuous time into mitigation strategies for unstable GD dynamics, by constructing novel learning rate schedules and regularisers that do not require additional hyperparameters. Like optimisation, smoothness regularisation is another pillar of deep learning's success with wide use in supervised learning and generative modelling. Despite their individual significance, the interactions between smoothness regularisation and optimisation have yet to be explored. We find that smoothness regularisation affects optimisation across multiple deep learning domains, and that incorporating smoothness regularisation in reinforcement learning leads to a performance boost that can be recovered using adaptions to optimisation methods.

==> dd_gan_explicit_regularisation.tex <==
\section{Connection to explicit regularisers}

The form of the modified losses that we have derived are related to explicit regularisers to stabilize adversarial training of GANs.
Consensus optimisation, SGDA, ODE-GAN and \citep{nagarajan2017gradient} are introducing explicit regularisation to reduce the strength
of the rotational field of the game or to stabilize training. While the form of the modified losses we introduce are similar, our use of explicit regularisation is only as a form to understand the effect of the implicit regularisers that we have found, rather than solving the aforementioned issues in GAN training. Cancelling the effect of implicit gradient regularisation is not sufficient, as can be seen by ODE-GAN, which still requires a regulariser despite not having first order regularisation effects. The arguments regarding the rotational field of the underlying game remain regardless of the integrator used - something that would need to be further analysed in the light of the implicit regularisation we have derived. We are making statements about the effect of discretisation on the underlying two player game, and notice its effects, rather than make statements about what regularisation is required given the underlying game. We should also make the difference between penalises which minimise your own norm, or penalise which minimise the norm of the other player - like discussed in~\citep{nagarajan2017gradient}, there is a connection there with unrolled GANs and increased stability.


The comparison between different methods is shown in Table~\ref{tab:methods_comp}.

\begin{table*}[h]
\centering
\begin{tabular}{ |c|c|c| }
 \hline
 Method & Discriminator ($\phi$) & Generator ($\theta$)\\
 \hline
 \hline
 IGR (A) & $- \frac {\lrp h}{4m}\norm{\nabla_{\phi} E}^2 + \frac{\lrp h}{4}\norm{\nabla_{\theta} E}^2$ & $ \frac{(2 \lrp - \lrt) h}{4}\norm{\nabla_{\phi} E}^2 + \frac{\lrt h}{4k}\norm{\nabla_{\theta} E}^2$  \\
 IGR (S) & $-h/4\norm{\nabla_{\phi} E}^2 + h/4\norm{\nabla_{\theta} E}^2$  & $-h/4\norm{\nabla_{\phi} E}^2 + h/4\norm{\nabla_{\theta} E}^2$ \\
 SGA/ACO (S) \citep{balduzzi2018mechanics} & - $\zeta sign(\nabla_{\phi} E,\nabla_{\phi}\norm{\nabla_{\phi} E}^2) \norm{\nabla_{\phi} E}^2$ &  $\zeta sign(\nabla_{\phi} E,\nabla_{\theta}\norm{\nabla_{\theta} E}^2) \norm{\nabla_{\theta} E}^2$ \\
 Consensus opt (S)\citep{mescheder2017numerics} & $-\zeta \norm{\nabla_{\phi} E}^2 - \zeta \norm{\nabla_{\theta} E}^2$ & $\zeta \norm{\nabla_{\phi} E}^2 + \zeta \norm{\nabla_{\theta} E}^2$ \\
Locally stable GAN (S) \citep{nagarajan2017gradient} & \text{\sffamily X} &  $\zeta \norm{\nabla_{\phi} E}^2$ \\
 ODE-GAN (S)& $ - \zeta \norm{\nabla_{\theta} E}^2$ &  \text{\sffamily X} \\
 \hline
\end{tabular}
\caption{Comparison with different methods in the zero sum case. We assume a $\min_{\theta} \max_{\phi}$ game, so we translate signs from the other papers (in case they use a min min or max max formulation). The learning rates assumed are $\lrp h$ and $\lrt h$ for the discriminator and generator, and the number of updates $m$ and $k$, respectively. $\zeta$ denotes the regularisation coefficient hyperparameter in methods which require one. S and A denote whether updates are simultaneous or alternating.}
\label{tab:methods_comp}
\end{table*}


Beyond this, add here a few other related works.


==> gc_mnist.tex <==
\subsection{MNIST results}
\label{sec:gc_appendix_mnist}

We present results on the MNIST dataset with explicit GC (Jacobian) regularisation in Figure~\ref{fig:explicit_gc_regularisation_mnist}, and results with $L_2$ regularisation, gradient norm regularisation and spectral regularisation on MNIST in Figures~\ref{fig:l2_regularisation_mnist}, ~\ref{fig:flatness_regularisation_mnist}, and~\ref{fig:spectral_regularisation_mnist} respectively; these results use a 4 layer MLP with 4 hidden layers with 200 neurons per layer on MNIST with learning rate of 0.02, batch size of 128, for 100000 steps. Results showing the implicit regularisation effect induced by large learning rates and small batch sizes are shown in Figures~\ref{fig:learning_rates_mnist} and \ref{fig:batch_sizes_mnist}; these results use 6 layers with 500 neurons, trained for 100000 steps.





 \begin{figure}[t]
  \centering
  \includegraphics[height=0.4\linewidth]{gc/explicit_gc_regularization_mnist}
    \includegraphics[height=0.4\linewidth]{gc/explicit_gc_regularization_mnist_accuracy}
  \caption[Jacobian (GC) explicit regularisation on MNIST.]{\textbf{Jacobian (GC) explicit regularisation}. Results obtained using 1 seed. }
  \label{fig:explicit_gc_regularisation_mnist}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=1
  \linewidth]{gc/learning_rates_mnist}
  \caption[Geometric complexity decreases with higher learning rates on MNIST.]{{\bf Geometric complexity decreases with higher learning rates on MNIST}. The batch size is 512. Results use 5 seeds.}
  \label{fig:learning_rates_mnist}
\end{figure}



\begin{figure}[h]
  \centering
  \includegraphics[width=1
  \linewidth]{gc/batch_sizes_mnist}
  \caption[Geometric complexity decreases with smaller batch sizes on MNIST.]{{\bf Geometric complexity decreases with smaller batch sizes on MNIST}. The learning rate used is $0.02$. Results use 5 seeds.}
  \label{fig:batch_sizes_mnist}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=1
  \linewidth]{gc/l2_regularization_mnist}
  \caption[Geometric complexity decreases with L2 regularisation on MNIST.]{{\bf Geometric complexity decreases with L2 regularisation on MNIST}. We regularised the loss by adding to it the L2 norm penalty $\zeta\sum_i \|W_i\|_F^2$ where $W_i$ are the layer weight matrices. Results use 5 seeds. }
  \label{fig:l2_regularisation_mnist}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=1
  \linewidth]{gc/spectral_regularization_mnist}
  \caption[Geometric complexity decreases with spectral regularisation on MNIST.]{{\bf Geometric complexity decreases with spectral regularisation on MNIST}. We regularized the loss by adding to it the spectral norm penalty $\zeta/2\sum_i \sigma_{\max}(W_i)^2$ where $W_i$ are the layer weight matrices as described in \cite{miyato2018spectral}. Results use 5 seeds.}
  \label{fig:spectral_regularisation_mnist}
\end{figure}


\begin{figure}[h]
  \centering
  \includegraphics[width=1
  \linewidth]{gc/flatness_regularization_mnist}
  \caption[Geometric complexity decreases with gradient norm regularisation on MNIST.]{{\bf Geometric complexity decreases with gradient norm regularisation on MNIST}. We regularized the loss by adding to it the gradient penalty $\zeta \|\nabla_\theta L_B(\theta)\|^2$ where $L_B$ is the batch loss. Results use 5 seeds.}
  \label{fig:flatness_regularisation_mnist}
\end{figure}

==> gd_dev_discrete_app.tex <==
\section{Derivation of gradient descent from an approximation perspective}

We can derive the gradient descent update from a discrete-time perspective, using the use of a Taylor expansion. 

\begin{align}
\min_{\vu}& E(\vtheta_{t-1} + \vu) \approx E(\vtheta_{t-1}) + \vu^T \nabla_{\vtheta} E(\vtheta_{t-1}) \\
s.t.& \norm{\vu}^2 \le \epsilon
\end{align}

thus if we introduce the Lagrange multiplier $\lambda$
we then have the KKT conditions with solution $\vu^*$:
\begin{align}
\nabla_{\vtheta} E(\vtheta_{t-1}) + 2 \lambda \vu^* &= 0 \\
\lambda (\norm{\vu^*}^2 - \epsilon) &= 0 \label{eq:min_kkt}
\end{align}

\begin{align}
\vu^* = -\frac{1}{2  \lambda} \nabla_{\vtheta} E(\vtheta_{t-1})
\end{align}

replacing this in Eq \eqref{eq:min_kkt}, we have:
\begin{align}
\norm{\vu^*} = \frac{1}{2 \lambda} \norm{\nabla_{\vtheta} E(\vtheta_{t-1})} = \sqrt \epsilon \implies \lambda = \frac{1}{2 \sqrt \epsilon} \norm{\nabla_{\vtheta} E(\vtheta_{t-1})}
\end{align}

leading to the solution
\begin{align}
\vu^* = -\frac{\sqrt \epsilon}{\norm{\nabla_{\vtheta} E(\vtheta_{t-1})}} \nabla_{\vtheta} E(\vtheta_{t-1})
\end{align}

This approach of deriving gradient descent showcases the connection between learning rates and gradient norms.

==> stability_analysis_derivation.tex <==
\section{Stability analysis derivation}

\label{sec:stability_analysis_derivation}

We now provide a justification for the stability analysis result we provided in Section~\ref{sec:stability_analysis_overview}. We start with a linearisation argument: consider a neighbourhood $\mathcal{U}$ such that $\vtheta^* \in \mathcal{U}$ and the linear approximation of $f(\vx) = f(\vtheta^*) + \jacthetaf(\vtheta^*) (\vtheta - \vtheta^*)=  \jacthetaf(\vtheta^*) (\vtheta - \vtheta^*)$ is exact. We note that this is not a formal argument, for a rigurous proof we rely on the Hartman–Grobman theorem~\citep{grobman,hartman1960lemma}. 

We then have:
\begin{align}
 \dot{\vtheta} = f(\vtheta) = \jacthetaf(\vtheta^*) (\vtheta - \vtheta^*)
\end{align}

leading to 
\begin{align}
 \dot{(\vtheta - \vtheta^*)} = f(\vtheta) = \jacthetaf(\vtheta^*) (\vtheta - \vtheta^*)
\end{align}

which is a linear system with the solution:
\begin{align}
\vtheta(t) = \vtheta^* + e^{\jacthetaf(\vtheta^*)t} (\vtheta(0) - \vtheta^*)
\end{align}

Thus to show exponential asymptotic convergence, we need to show that $\lim_{t \rightarrow \infty}  e^{\jacthetaf(\vtheta^*)t} (\vtheta(0) - \vtheta^*) = 0$ and it does so at an exponential rate. To do so, we have to use the assumption that  $\jacthetaf(\vtheta^*)$ only has eigenvalues with negative real part.
Since $\jacthetaf(\vtheta^*)$ need not be symmetric, its eigenvalues can be complex. We then rely on the Jordan normal form of $\jacthetaf(\vtheta^*)$ and write:
\begin{align}
\jacthetaf(\vtheta^*) = P^{-1} J P
\end{align}

where $J$ is a block diagonal matrix 
\begin{align}
J = \begin{bmatrix}
{J_0} & \hdots & 0 & 0\\
0 & {J_1} & \hdots & 0 \\
\vdots &  &  & \vdots \\
 0 & \hdots & 0 & {J_{m}}\\
\end{bmatrix} 
\end{align}
Each block $J_k$ corresponds to a unique eigenvalue $\lambda_k$ with duplicity $n_k$, with $J_k \in \mathbb{C}^{n_k, n_k}$ where
\begin{align}
 J_{k} = \lambda_k I_{n_k} + Z_{n_k}
\end{align}

where $ I_{n_k}$ is the identity matrix of dimension $n_k$ and $Z_{n_k}$ is a matrix with all $0$s apart from one off diagonal:
\begin{align}
Z_{n_k} = \begin{bmatrix}
0 & 1&  \hdots & 0 & 0 \\
0 & 0&  1 & \hdots & 0 \\
\vdots & \vdots& \ddots & \ddots &  \vdots\\
0 & 0 & 0 & \hdots & 1 \\
0 & 0 & 0 & 0 & 0
\end{bmatrix}
\label{eq:z_structure}
\end{align}

We have that
\begin{align}
e^{\jacthetaf(\vtheta^*) t} &= e^{P^{-1} J P t} = \sum_{i=0}^{\infty} \frac{1}{i!} (P^{-1} Jt P)^i \\ 
                                 &=  \sum_{i=0}^{\infty} \frac{1}{i!} P^{-1} (Jt)^i P= P^{-1} \left(\sum_{i=0}^{\infty} \frac{1}{i!} (Jt)^i\right) P = P^{-1}e^{Jt}  P 
\end{align}

and thus
\begin{align}
 \norm{e^{\jacthetaf(\vtheta^*)t} (\vtheta(0) - \vtheta^*)}_F &\le \norm{{P^{-1}e^{Jt}  P }}_F \norm{(\vtheta(0) - \vtheta^*)}_F \\
 &\le \norm{e^{Jt}}_F\norm{P^{-1}}_F \norm{P}_F \norm{(\vtheta(0) - \vtheta^*)}_F
 \label{eq:stability_analysis_norm}
\end{align}

We are thus left with the task of bounding $\norm{e^{Jt}}$. Since $J$ is a block-diagonal matrix and thus its structure is preserved under addition and multiplication, if we use the Taylor expansion of the exponential we can write:
\begin{align}
e^{Jt} = \begin{bmatrix}
e^{J_0 t} & \hdots & 0 & 0\\
0 & e^{J_1 t} & \hdots & 0 \\
\vdots &  &  & \vdots \\
 0 & \hdots & 0 & e^{J_{m} t}\\
\end{bmatrix} 
\end{align}

If we consider the Frobenius norm, we have
\begin{align}
\norm{e^{J t}}^2_F = \sum_{i=1}^{m} \norm{e^{J_m t} }^2_F \le m \norm{e^{J_k t}}^2_F
\label{eq:e_j_bound}
\end{align}

where $J_k$ is the block with the maximum Frobenius norm in $J$. Now using the form of $J_k$ we have:

\begin{align}
\norm{e^{J_k t}}_F = \norm{e ^{\lambda_k t I + t Z_{n_k}}}_F = \norm{e ^{t \lambda_k I}_F e^ {t Z_{n_k}}}_F
 \le \norm{e ^{t \lambda_k I}}_F \norm{e^{ t Z_{n_k}}}_F
\end{align}

Using the form of $Z_{n_k}$ in Eq~\eqref{eq:z_structure} we have that
\begin{align}
e^{t Z_{n_k}} = \sum_{i=0}^{\infty} \frac{1}{i!}{(t Z_{n_k})}^i = \sum_{i=0}^{n_k} \frac{1}{i!}{ (t Z_{n_k})}^i
\end{align}

since ${Z_{n_k}}^i =0$ for $i \ge {n_k}$. We thus can treat $\norm{e^ {Z_{n_k}}}_F$ which we denote as $C$. We then have:
\begin{align}
\norm{e^{J_k t} }_F \le C \norm{e ^{t \lambda_k I}}_F
\label{eq:j_k_bound}
\end{align}{}

If we use the assumption that $\lambda_k$ has negative real part we have $\lambda_k = -x + i y$ with $x > 0$ and:
\begin{align}
\norm{e ^{t \lambda_k I}}_F = \sqrt{n_k} \norm{e ^{t \lambda_k}}_F  = \sqrt{n_k} \norm{e ^{-x  t+ i t y}}_F \le  \sqrt{n_k} \norm{e ^{-x t}}_F \norm{e ^{i t y}}_F 
\label{eq:lambda_k_bound}
\end{align}

Thus from Eqs~\eqref{eq:j_k_bound} and~\eqref{eq:lambda_k_bound} we have:
\begin{align}
\norm{e^{t J_k}}_F \le C n_k e ^{-t x}
\end{align}

with $x = \Re(\lambda_k)$. Replacing back in Eq~\eqref{eq:e_j_bound} we have:
\begin{align}
\norm{e^{J t}}_F \le \sqrt{m n_k} C e ^{-t x}
\end{align}

Replacing back in Eq~\eqref{eq:stability_analysis_norm} leads to:
\begin{align}
 \norm{e^{\jacthetaf(\vtheta^*)t} (\vtheta(0) - \vtheta^*)}_F 
 &\le \norm{e^{t J} }_F\norm{P^{-1}}_F \norm{P}_F \norm{(\vtheta(0) - \vtheta^*)}_F \\
 &\le  \sqrt{m n_k} C e ^{-t x} \norm{P^{-1}}_F \norm{P}_F \norm{(\vtheta(0) - \vtheta^*)}_F \\
 &\le K e ^{- t x} \norm{(\vtheta(0) - \vtheta^*)}_F
\end{align}

with $x > 0$ which concludes the proof.






